Prophet Matching Meets Probing with Commitment

We consider the online stochastic matching problem for bipartite graphs where edges adjacent to an online node must be probed to determine if they exist, based on known edge probabilities. Our algorithms respect commitment, in that if a probed edge exists, it must be used in the matching. We study this matching problem subject to a downward-closed constraint on each online node's allowable edge probes. Our setting generalizes the commonly studied patience (or time-out) constraint which limits the number of probes that can be made to an online node's adjacent edges. We introduce a new LP that we prove is a relaxation of an optimal offline probing algorithm (the adaptive benchmark) and which overcomes the limitations of previous LP relaxations. (1) A tight $\frac{1}{2}$ ratio when the stochastic graph is generated from a known stochastic type graph where the $t^{th}$ online node is drawn independently from a known distribution $\scr{D}_{\pi(t)}$ and $\pi$ is chosen adversarially. We refer to this setting as the known i.d. stochastic matching problem with adversarial arrivals. (2) A $1-1/e$ ratio when the stochastic graph is generated from a known stochastic type graph where the $t^{th}$ online node is drawn independently from a known distribution $\scr{D}_{\pi(t)}$ and $\pi$ is a random permutation. We refer to this setting as the known i.d. stochastic matching problem with random order arrivals. Our results improve upon the previous best competitive ratio of $0.46$ in the known i.i.d. setting against the standard adaptive benchmark. Moreover, we are the first to study the prophet secretary matching problem in the context of probing, where we match the best known classical result.

==> new-abstract <==
\begin{abstract}


 
Within the context of stochastic probing with commitment, we consider
the online stochastic matching problem for bipartite graphs where edges adjacent to an online node must be probed to
determine if they exist, based on known edge probabilities. If a probed edge
exists, it must be used in the matching (if possible). In addition to improving upon existing stochastic bipartite matching results, our results can also be seen as extensions to multi-item prophet inequalities. We study this matching problem for given  constraints on the allowable sequences of probes adjacent to an online node. Our setting generalizes the patience (or time-out) constraint  which limits the number of probes that can be made to edges. The generality of our setting leads to some  modelling and computational efficiency issues that are not encountered in previous works. To resolve these issues, we introduce a new LP that we prove is a relaxation of an optimal offline benchmark and  overcomes the limitations of previous LP relaxations. We establish new competitive bounds
all of which generalize the standard non-probing  setting when edges do not need to be probed (i.e., exist with certainty). 
Specifically, we establish the following competitive ratio results for a  general formulation of edge probing constraints, arbitrary edge weights, and arbitrary edge probabilities:

\begin{enumerate}
 
\item A tight  $\frac{1}{2}$ ratio when the stochastic graph is generated from a known stochastic type graph where the $\pi(i)^{th}$ online node is drawn independently from a known  distribution $\scr{D}_{\pi(i)}$ and $\pi$ is chosen adversarially. We refer to this setting as the known i.d. stochastic matching problem with adversarial arrivals. 
\item A $1-1/e$ ratio when the stochastic graph is generated from a known stochastic type graph where the $\pi(i)^{th}$ online node is drawn independently from a  known distribution $\scr{D}_{\pi(i)}$ and $\pi$ is a random permutation. This is referred to as the known i.d. stochastic matching problem with random order arrivals. 
\end{enumerate}

We note that the known i.d. model generalizes the more common online  stochastic matching  model where the stochastic graph (but not the edge probabilities nor the order of online arrivals)  is known in advance to the algorithm. Our i.d. model also  generalizes the prophet inequality and prophet secretary  
models  to the probing setting. Our competitive ratios are established by a olynomial time algorithm in the context of general probing constraints including  matroid and budget (equivalently, knapsack) constraints.  

%In deriving our results, we clarify and expand upon previous offline benchmarks, relative to which one defines an appropriate definition of the competitive ratio.
%In particular, we introduce a new LP relaxation which upper
%bounds the performance of ``an  optimum offline  probing algorithm''. 
%This new LP  allows us to overcome some previous negative results (i.e. stochasticity gaps).  
%While this LP has exponentially
%many variables, it has polynomially many constraints
%and we show how it can be solved efficiently (i.e., in polynomial time) under some mild assumptions on the edge probing constraints.
\end{abstract}



